Performance Analysis of Decentralized Physical Infrastructure Networks and Centralized Clouds

The advent of Decentralized Physical Infrastructure Networks (DePIN) represents a shift in the digital infrastructure of today's Internet. While Centralized Service Providers (CSP) monopolize cloud computing, DePINs aim to enhance data sovereignty and confidentiality and increase resilience against a single point of failure. Due to the novelty of the emerging field of DePIN, this work focuses on the potential of DePINs to disrupt traditional centralized architectures by taking advantage of the Internet of Things (IoT) devices and crypto-economic design in combination with blockchains. This combination yields Acurast, a more distributed, resilient, and user-centric physical infrastructure deployment. Through comparative analysis with centralized systems, particularly in serverless computing contexts, this work seeks to lay the first steps in scientifically evaluating DePINs and quantitatively comparing them in terms of efficiency and effectiveness in real-world applications. The findings suggest DePINs' potential to (i) reduce trust assumptions and physically decentralized infrastructure, (ii) increase efficiency and performance simultaneously while improving the computation's (iii) confidentiality and verifiability.

==> assets/4-eval-fig-performance.tex <==
\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[
    xlabel={Time [s]},
    ylabel={System Resource Usage [\%]},
    xmin=200, xmax=500,
    ymin=0, ymax=130,
    xtick={250, 350, 450},
    ytick={0, 25, 50, 75, 100},
    legend pos=north east,
    width=\linewidth,
    legend cell align={left},
    height=4.8cm,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    ]
    coordinates {
    (0,25)(14,17)(28,25)(42,23)(56,21)(70,21)(84,18)(98,23)(112,23)(126,25)(140,14)(154,18)(168,25)(182,19)(196,19)(210,23)(224,26)(238,19)(252,43)(266,94)(280,93)(294,76)(308,84)(322,75)(336,79)(350,76)(364,75)(378,50)(392,27)(406,23)(420,25)(434,21)(448,23)(462,26)(476,22)(490,24)(504,21)(518,21)(532,23)(546,25)(560,24)(574,21)(588,23)(602,24)(616,28)(630,20)(644,16)(658,22)(672,28)(686,16)(700,17)(714,24)(728,22)(742,20)(756,24)(770,25)(784,24)(798,17)(812,22)(826,23)(840,29)(854,21)(868,20)(882,26)(896,19)(910,25)(924,29)(938,26)(952,24)(966,27)(980,25)(994,19)(1008,18)(1022,23)(1036,19)
    };
    \addlegendentry{CPU}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    dashed
    ]
    coordinates {
    (0,9.37303899310746)(14,9.38946681019749)(28,9.37099827048758)(42,9.38446703977879)(56,9.51599161263003)(70,9.45364753659271)(84,9.44334188736232)(98,9.44436224867225)(112,9.44436224867225)(126,9.45395364498569)(140,9.45130070557985)(154,9.44650500742313)(168,9.44956609135295)(182,9.45558622308159)(196,9.46997331755175)(210,9.5131346009622)(224,9.51395089001015)(238,9.53027667096919)(252,9.62986393481932)(266,9.84036447305991)(280,9.89556601992766)(294,9.89668841736859)(308,9.91556510160248)(322,9.96199154120474)(336,9.81689616293129)(350,9.81618191001434)(364,9.81546765709738)(378,9.80720273048687)(392,9.63588406654796)(406,9.62241529725676)(420,9.62302751404272)(434,9.63231280196318)(448,9.62996597095031)(462,9.59200853022055)(476,9.62578248957956)(490,9.62221122499477)(504,9.60772209439363)(518,9.61904810493396)(532,9.62282344178073)(546,9.6165992377901)(560,9.61966032171992)(574,9.62568045344857)(588,9.61221168415736)(602,9.61884403267197)(616,9.6115994673714)(630,9.61843588814799)(644,9.61251779255034)(658,9.62149697207781)(672,9.61731349070706)(686,9.60496711885679)(700,9.59211056635155)(714,9.59374314444745)(728,9.59935513165212)(742,9.58343749521706)(756,9.5910902050416)(770,9.61476258743221)(784,9.60068160135504)(798,9.60047752909305)(812,9.61976235785092)(826,9.60588544403573)(840,9.60792616665561)(854,9.60088567361703)(868,9.5996612400451)(882,9.61976235785092)(896,9.60690580534567)(910,9.60751802213164)(924,9.60915060022754)(938,9.60353861302287)(952,9.60119178201001)(966,9.60945670862052)(980,9.58935559081471)(994,9.5997632761761)(1008,9.5860904346229)(1022,9.61904810493396)(1036,9.61068114219245)
    };
    \addlegendentry{RAM}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    mark=square
    ]
    coordinates {
    (0,0)(14,0)(28,0)(42,0)(56,0)(70,0.17574692442882248)(84,0)(98,0)(112,0)(126,0)(140,0)(154,0)(168,0)(182,0)(196,0)(210,0)(224,0)(238,0)(252,0)(266,0.4393673110720563)(280,0)(294,0)(308,18.36555360281195)(322,5.623901581722319)(336,0)(350,0)(364,0)(378,0)(392,0)(406,0)(420,0)(434,0)(448,0)(462,0)(476,0)(490,0)(504,0)(518,0)(532,0)(546,0)(560,0)(574,0)(588,0)(602,0)(616,0)(630,0)(644,0)(658,0)(672,0)(686,0)(700,0)(714,0)(728,0)(742,0)(756,0)(770,0)(784,0)(798,0)(812,0)(826,0)(840,0)(854,0)(868,0)(882,0)(896,0)(910,0)(924,0)(938,0)(952,0)(966,0)(980,0)(994,0)(1008,0)(1022,0)(1036,0)(1050,0)
    };
    \addlegendentry{Disk Read}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    mark=triangle,
    ]
    coordinates {
    (0,0.4959159859976663)(14,0)(28,0.10210035005834306)(42,0.05834305717619603)(56,0.1750291715285881)(70,0)(84,0)(98,0.08751458576429405)(112,0)(126,0)(140,0)(154,0)(168,0)(182,0)(196,0)(210,0)(224,0.08751458576429405)(238,0.043757292882147025)(252,0)(266,0.1750291715285881)(280,0.1896149358226371)(294,12.310385064177364)(308,0)(322,0)(336,16.525670945157525)(350,0.043757292882147025)(364,0)(378,0)(392,0)(406,0)(420,0)(434,0)(448,0)(462,0)(476,0)(490,0)(504,0)(518,0)(532,0)(546,0)(560,0)(574,0)(588,0)(602,0)(616,0)(630,0)(644,0)(658,0)(672,0)(686,0)(700,0)(714,0)(728,0)(742,0)(756,0)(770,0)(784,0)(798,0)(812,0)(826,0)(840,0)(854,0)(868,0)(882,0)(896,0)(910,0)(924,0)(938,0)(952,0)(966,0)(980,0)(994,0)(1008,0)(1022,0)(1036,0)(1050,0)
    };
    \addlegendentry{Disk Write}
    
   \draw[blue] (axis cs: 251,0) -- 
       (axis cs: 251,85)node[anchor=center, above=0.5pt]{\small{(1)}};
   \draw[blue] (axis cs: 265,0) -- 
       (axis cs: 265,105)node[anchor=center, above=0.5pt]{\small{(2)}};
   \draw[blue] (axis cs: 341,0) -- 
       (axis cs: 341,100)node[anchor=center, above=0.5pt]{\small{(3)}};
    
    
\end{axis}
\end{tikzpicture}
\caption{Device Resource Impact}
\label{fig:ransomware}
\end{figure}

==> assets/4-histogram-aws.tex <==


%\begin{figure}
%    \centering

\begin{tikzpicture}
\begin{axis}[
    height=4.8cm,
    width=8cm,    
    ybar,
    ymin=0,
    xlabel={Response Time [ms]},
    ylabel={Frequency},
    xtick={3400, 3800, 4200, 4600}
]

\addplot +[
    hist={
        bins=30,
        data min=3300,
        data max=4500
    }
] table [y index=0] {aws.csv};
    
\draw[blue] (axis cs: 3340,0) -- 
       (axis cs: 3340,80)node[anchor=center, above=0.5pt]{\small{min}};
\draw[blue] (axis cs: 4487,0) -- 
       (axis cs: 4487,80)node[anchor=center, above=0.5pt]{\small{max}};
\draw[blue] (axis cs: 3738,0) -- 
       (axis cs: 3738,80)node[anchor=center, above=0.5pt]{\small{med}};
\end{axis}
\end{tikzpicture}
%    \caption{AWS}
%    \label{fig:enter-label}
%\end{figure}

==> assets/4-histogram-azure.tex <==


%\begin{figure}
%    \centering

\begin{tikzpicture}
\begin{axis}[
    height=4.8cm,
    width=8cm,    
    ybar,
    ymin=0,
    xlabel={Response Time [ms]},
    ylabel={Frequency},
    xtick={6000, 6800, 7600, 8400}
]

\addplot +[
    hist={
        bins=30,
        data min=5757,
        data max=8379
    }   
] table [y index=0] {azure.csv};
    
\draw[blue] (axis cs: 5757,0) -- 
       (axis cs: 5757,30)node[anchor=center, above=0.5pt]{\small{min}};
\draw[blue] (axis cs: 8379,0) -- 
       (axis cs: 8379,30)node[anchor=center, above=0.5pt]{\small{max}};
\draw[blue] (axis cs: 6032,0) -- 
       (axis cs: 6032,30)node[anchor=center, above=0.5pt]{\small{med}};
\end{axis}
\end{tikzpicture}
 %   \caption{Azure}
 %   \label{fig:enter-label}
%\end{figure}

==> assets/4-histogram-sol.tex <==



\begin{tikzpicture}
\begin{axis}[
    height=4.8cm,
    width=8cm,    
    ybar,
    ymin=0,
    xlabel={Response Time [ms]},
    ylabel={Frequency},
    xtick={2400, 2700, 3000, 3300}
]

\addplot +[
    hist={
        bins=30,
        data min=2400,
        data max=3300
    }   
] table [y index=0] {sol.csv};
    
\draw[blue] (axis cs: 2473,0) -- 
       (axis cs: 2473,15)node[anchor=center, above=0.5pt]{\small{min}};
\draw[blue] (axis cs: 3138,0) -- 
       (axis cs: 3138,15)node[anchor=center, above=0.5pt]{\small{max}};
\draw[blue] (axis cs: 2785,0) -- 
       (axis cs: 2785,15)node[anchor=center, above=0.5pt]{\small{med}};
\end{axis}
\end{tikzpicture}

==> assets/4-histograms-gcp.tex <==


\begin{tikzpicture}
\begin{axis}[
    height=4.8cm,
    width=8cm,    
    ybar,
    ymin=0,
    xlabel={Response Time [ms]},
    ylabel={Frequency},
    xtick={5000, 6000, 7000, 8000}
]

\addplot +[
    hist={
        bins=30,
        data min=4700,
        data max=8000
    }   
] table [y index=0] {gcp.csv};
    
\draw[blue] (axis cs: 4732,0) -- 
       (axis cs: 4732,45)node[anchor=center, above=0.5pt]{\small{min}};
\draw[blue] (axis cs: 7980,0) -- 
       (axis cs: 7980,45)node[anchor=center, above=0.5pt]{\small{max}};
\draw[blue] (axis cs: 5686,0) -- 
       (axis cs: 5686,45)node[anchor=center, above=0.5pt]{\small{med}};
\end{axis}
\end{tikzpicture}
